Structural Resolution for Abstract Compilation of Object-Oriented Languages

We propose abstract compilation for precise static type analysis of object-oriented languages based on coinductive logic programming. Source code is translated to a logic program, then type-checking and inference problems amount to queries to be solved with respect to the resulting logic program. We exploit a coinductive semantics to deal with infinite terms and proofs produced by recursive types and methods. Thanks to the recent notion of structural resolution for coinductive logic programming, we are able to infer very precise type information, including a class of irrational recursive types causing non-termination for previously considered coinductive semantics. We also show how to transform logic programs to make them satisfy the preconditions for the operational semantics of structural resolution, and we prove this step does not affect the semantics of the logic program.

==> eptcsdata.tex <==
\providecommand{\firstpage}{19}
\providecommand{\publicationstatus}{E. Komendantskaya and J. Power (Eds.):\\ Coalgebra, Horn Clause Logic Programming and Types\\
EPTCS 258, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.258.2}{10.4204/EPTCS.258.2}}
\pdfoutput=1

